The OS* Algorithm: a Joint Approach to Exact Optimization and Sampling

Most current sampling algorithms for high-dimensional distributions are based on MCMC techniques and are approximate in the sense that they are valid only asymptotically. Rejection sampling, on the other hand, produces valid samples, but is unrealistically slow in high-dimension spaces. The OS* algorithm that we propose is a unified approach to exact optimization and sampling, based on incremental refinements of a functional upper bound, which combines ideas of adaptive rejection sampling and of A* optimization search. We show that the choice of the refinement can be done in a way that ensures tractability in high-dimension spaces, and we present first experiments in two different settings: inference in high-order HMMs and in large discrete graphical models.

==> Background.tex <==
\subsection{Background}
\label{sec:background}


% \begin{figure*}
% \centering{\includegraphics[clip=true, draft=false, trim=0cm 5.5cm 0cm 6cm, scale=.45]{FIGS/RS1-ARS1}}
% \caption{Rejection Sampling (left); Adaptive Rejection Sampling in one dimension (right).}
%  	\label{fig:RS1-ARS1}
% \end{figure*}

Let $\p:X\rightarrow \mathbb{R}_{+}$ be a measurable $L_1$ function with respect to a base measure $\mu$ on a space $X$, i.e. 
$\int_X p(x) d\mu(x) < \infty$.  We define $\pbar(x) \equiv \frac{\p(x)}{\int_X p(x) d\mu(x)}$. The function \p can be seen as an unnormalized density over $X$, and $\pbar$ as a normalized density which defines a probability distribution over $X$, called the \emph{target distribution}, from which we 
want to sample from\footnote{By abuse of language, we will also say that a sample from $\pbar$ is a sample from $\p$.}. While we may not be able to sample directly from the target distribution $\pbar$, let us assume that we can easily compute $p(x)$ for any given $x$. 
\emph{Rejection Sampling} (RS) \cite{Robert2004} then works as follows. We define a certain unnormalized \emph{proposal density} $\q$ over $X$, which is such that (i) we know how to directly sample from it (more precisely, from $\qbar$), and (ii) $q$ dominates $p$, i.e. for all $x\in X, p(x) \leq q(x)$. We then repeat the following process: (1) we draw a sample $x$ from $q$, (2) we compute the ratio $r(x)\equiv p(x)/q(x) \leq 1$, (3) with probability $r(x)$ we accept $x$, otherwise we reject it, (4) we repeat the process with a new $x$. It can then be shown that this procedure produces an exact sample from $\p$. Furthermore, the average rate at which it produces these samples, the \emph{acceptance rate}, is equal to $P(X)/Q(X)$ \cite{Robert2004}, where for a (measurable) subset $A$ of $X$, we define $P(A) \equiv \int_A p(x) d\mu(x)$ and similarly with $Q$. In Fig.~\ref{fig:RS1-ARS1} (left), the acceptance rate is equal to the ratio of the area below the $p$ curve with that below the $q$ curve.



\begin{figure}[H]
\includegraphics[clip=true, draft=false, trim=6cm 6cm 3cm 7cm, scale=.55]{RS1}
\caption{Rejection Sampling}
	\label{fig:RS1}
\end{figure}


% \begin{figure}[H]
% \centering{\includegraphics[clip=true, draft=false, trim=6cm 6cm 6cm % 5cm, scale=.6]{FIGS/ARS1}}
% \caption{ ARS}
% 	\label{fig:ARS1}
% \end{figure}




% \begin{comment}
% {\sl Our own previous ID recently introduced a way to do adaptive % rejection sampling in higher dimensional, and also, especially, % discrete spaces, which we called \ARSstar, based on analogies with the % \Astar optimization method. The main idea of \ARSstar can be % illustrated by the following figure.}
% \begin{figure}[H]
% \centering{\includegraphics[clip=true, draft=false, trim=6cm 5cm 6cm % 5cm, scale=.6]{FIGS/ARSstar1}}
% \caption{\ARSstar}
% 	\label{fig:ARSstar1}
% \end{figure}

% In this figure, $q_0$ represents an initial proposal density, which is % a constant upper bound to $p$ everywhere over $X$, where $(X,\mu)$ is % an arbitrary measure space.\footnote{We can always assume that $q_0$ % is a constant function,  by the following trick: for any target % $\tilde{p}$ and any $\tilde{q}$ larger than $\tilde{p}$ which is of % finite mass relative to a base measure $\tilde{\mu}$ (e.g. with % $\int_X \tilde{q}(x) d\tilde{\mu} (x) < \infty$), we can recalibrate % the base measure $\tilde{\mu}$ into the measure $\mu \equiv % \tilde{q}.\tilde{\mu}$, which corresponds to recalibrating the density % $\tilde{p}$ into $p \equiv \tilde{p}/\tilde{q}$ and the density % $\tilde{q}$ into $q_0 \equiv \tilde{q}/\tilde{q} = 1 = constant$.}
% We start by sampling with $q_0$, then on a first reject somewhere in % $X$, we split the space $X$ into two subspaces $X_1,X_2$ (informally % represented in the figure by the left and right halves of the line % representing $X$), and now use the fact that we have a finer partition % of $X$ to update our upper bound $q_0$ over $X$ into a finer upper % bound on $X_1$ and a finer upper bound on $X_2$, resulting then in new % upper bound $q_1$ over the whole of $X$.  We then sample using $q_1$, % and experience at some time another reject, say on a point of $X_1$; % we then partition $X_1$ into two parts $X_{11}$ and $X_{12}$, refine % the bounds on these parts, and iterate this process until we observe % an acceptance rate above a certain predefined threshold.
% The \ARSstar ID gave several examples of the application of this % technique --- using a somewhat different, but equivalent, presentation % --- to continuous and to discrete sampling, which we do not re-state % here.
% \end{comment}

==> Experiments.tex <==
\section{Experiments}\label{sec:experiments}
\label{sec:experiments}

\input{ExperimentsHMM.tex}

\input{ExperimentsGraphical.tex}





